Joint distribution of Busemann functions in the exactly solvable corner growth model

The 1+1 dimensional corner growth model with exponential weights is a centrally important exactly solvable model in the Kardar-Parisi-Zhang class of statistical mechanical models. While significant progress has been made on the fluctuations of the growing random shape, understanding of the optimal paths, or geodesics, is less developed. The Busemann function is a useful analytical tool for studying geodesics. This paper describes the joint distribution of the Busemann functions, simultaneously in all directions of growth. As applications of this description we derive a marked point process representation for the Busemann function across a single lattice edge and calculate some marginal distributions of Busemann functions and semi-infinite geodesics.

==> LouisTimoDefs.tex <==

\usepackage{amsmath,amssymb,amsthm,tikz,mathrsfs,mathabx}
\RequirePackage[numbers,sort&compress]{natbib}
\usepackage{scalerel}    %%%%  used first for scaling \bullet for missing argument in a function 
\usepackage{stmaryrd}   %%%% for integer interval notation, though I also have my own    

\usepackage{comment,placeins} % added by Louis
\usepackage{mathdots} 
%\usepackage{newpxmath,newpxtext}
% new \oset macro
\makeatletter
\newcommand{\oset}[3][0ex]{%
	\mathrel{\mathop{#3}\limits^{
			\vbox to#1{\kern-1\ex@
				\hbox{$\scriptstyle#2$}\vss}}}}
\makeatother


%\usepackage[colorlinks]{hyperref}  

\usepackage{graphicx,tikz,subfigure,color}
\usetikzlibrary{decorations.pathreplacing}
\usepackage{datetime2}

\RequirePackage{color}
\RequirePackage[colorlinks, urlcolor=my-blue,linkcolor=my-link,citecolor=my-green]{hyperref}
\definecolor{my-link}{rgb}{0.5,0.0,0.0}
\definecolor{my-blue}{rgb}{0.0,0.0,0.6}
\definecolor{my-red}{rgb}{0.5,0.0,0.0}
\definecolor{my-green}{rgb}{0.0,0.5,0.0}
\definecolor{nicos-red}{rgb}{0.75,0.0,0.0}
\definecolor{light-gray}{gray}{0.6}
\definecolor{really-light-gray}{gray}{0.8}

\usepackage{nicefrac}
\usepackage{enumerate}
%\usepackage{wasysym}

%Command to not generate a shitload of files
%\nofiles


%%%%%%%%
\addtolength{\hoffset}{-.8in} 
\addtolength{\textwidth}{1.6in}
\addtolength{\voffset}{-.4in} 
%\addtolength{\footskip}{.3in}
%\setlength{\oddsidemargin}{0in}
%\setlength{\evensidemargin}{0in}
%\setlength{\footskip}{0.2in}
%\setlength{\topmargin}{0.5in}
\addtolength{\textheight}{.7in}
%\baselineskip=12pt   %%seems to make no difference? 
\linespread{1.1}     %this works nicely to produce a more readable cropped 2-1


\newtheorem{theorem}{\sc Theorem}[section]
\newtheorem{lemma}[theorem]{\sc Lemma}
\newtheorem{proposition}[theorem]{\sc Proposition}
\newtheorem{corollary}[theorem]{\sc Corollary}
\newtheorem{assumption}[theorem]{\bf Assumption}
\newtheorem{definition}[theorem]{\it Definition}
%\newtheorem{remark}[theorem]{\sc Remark}
\numberwithin{equation}{section}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}


\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\nn}{\nonumber}
\providecommand{\abs}[1]{\vert#1\vert}
\providecommand{\norm}[1]{\Vert#1\Vert}
\providecommand{\pp}[1]{\langle#1\rangle}
\newcommand{\fl}[1]{\lfloor{#1}\rfloor} 
\newcommand{\ce}[1]{\lceil{#1}\rceil}

%%generic definitions 
\def\Coc{\mathscr K}
\def\Cor{\Coc_0}
\def\cC{\mathcal{C}}  \def\cD{\mathcal{D}}
\def\cF{\mathcal{F}}   \def\cE{\mathcal{E}}
\def\cG{\mathcal{G}}   \def\cW{\mathcal{W}}
\def\cH{\mathcal{H}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cP{\mathcal{P}}
\def\cR{\mathcal{R}}
\def\cU{\mathcal{U}}
\def\cS{\mathcal{S}}  \def\cT{\mathcal{T}}
\def\cI{\mathcal{I}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}  \def\cX{\mathcal{X}}   \def\cY{\mathcal{Y}}
\def\xhat{\hat x}
\def\wg{\eta}
\def\wgtil{\tilde\wg}
\def\esssup{\mathop{\mathrm{ess\,sup}}}
\def\gr{\mathcal G}
%\font \mymathbb = bbold10 at 11pt
\def\Hbar{\overline H}
\def\Hhat{\hat H}
\def\Phat{\widehat\P}
\def\Omhat{\widehat\Omega}
\def\kShat{\widehat\kS}
\def\That{\hat T}
\def\Bhat{\hat B}
\def\Vhat{\hat V}
\def\wzhat{\hat\wz}
\def\what{\hat\w}
\def\xbar{\bar x}
\def\t{\mathfrak t}
\def\tmin{{\underline\t}}
\def\tmax{{\bar\t}}

%\newcommand{\one}{{{\rm 1\mkern-2.1mu}\!{\rm I}}}
\newcommand{\one}{\mbox{\mymathbb{1}}}


\def\kS{\mathfrak{S}}

\def\bB{\mathbb{B}}\def\bD{\mathbb{D}}
\def\bE{\mathbb{E}}
\def\bL{\mathbb{L}}
\def\bN{\mathbb{N}}
\def\bP{\mathbb{P}}
\def\bQ{\mathbb{Q}}
\def\bR{\mathbb{R}}
\def\bZ{\mathbb{Z}}
\def\Zb{\mathbb{Z}}
\def\bI{\mathbb{I}}

\def\bS{\mathbb{S}}
 \def\Z{\bZ} \def\Q{\bQ} \def\R{\bR}\def\N{\bN}
  \def\evec{\mathbf{e}}\def\vvec{\mathbf{v}}   \def\uvec{\mathbf{u}}

\def\ntil{\tilde{n}}
\def\xtil{\tilde{x}}
\def\xvec{\mathbf{x}}
\def\yvec{\mathbf{y}}
\def\zvec{\mathbf{z}}
\def\Yvec{\mathbf{Y}}  \def\Zvec{\mathbf{Z}} \def\thvec{\boldsymbol{\theta}}
\def\qbar{\bar{q}}
\def\Ybar{\overline{Y}}
\def\w{\omega}
\def\om{\omega}
\def\taubar{\bar{\tau}}
\def\omvec{\bar\omega}
\def\psibar{\overline\psi} 
\def\e{\varepsilon}
\def\ind{\mathbf{1}}
\def\ddd{\displaystyle} 
\def\ri{{\mathrm{ri\,}}}

\def\mE{\mathbf{E}}   
\def\mH{\mathbf{H}}
\def\mP{\mathbf{P}}
\def\m1{\mathbf{1}}
\def\Ustat{\theta}
\def\Vstat{\rho}
\def \sqn{\sqrt{n}}
\def\kS{\mathfrak S}
  \DeclareMathOperator{\refl}{\rho} % reflection of a sequence across the index 0

\DeclareMathOperator{\Var}{Var}   \DeclareMathOperator{\Cov}{Cov}  
%%new def's 
 \def\Vvv{{\rm\mathbb{V}ar}}  \def\Cvv{{\rm\mathbb{C}ov}} 
 \def\hfun{h}
 \def\cJ{\mathcal{J}}  
 \def\wt{\widetilde}  \def\wh{\widehat} \def\wb{\overline} \def\wc{\widecheck}   \def\ul{\underline} 
 \def\qvar{\sigma_0}
  \def\chfn{\lambda}  %%char function
 \def\bT{\mathbb{T}} 
 
%%notation specific to this material 
\def\E{\bE}
\def\P{\bP} %% environment measure 
\def\wlev{\omvec} %environment at a level 
\def\shift{\theta}  %spatial shift  
\def\nbhd{\cR}  %set of admissible steps 
\def\jump{v} %jump variable chosen from transition for couplings
\def\flux{H}   %macroscopic flux
\def\vva{v_0} \def\vvb{v_1}   %%%intersections at level j 
\def\north{S_{\mathcal N}}  \def\south{S_{\mathcal S}}  \def\east{S_{\mathcal E}}  
\def\west{S_{\mathcal W}}  
 
\def\OSP{(\Omega, \kS, \P)}
\def\backpi{\overleftarrow{\mathbf{x}}} 
\def\backx{\overleftarrow{x}}
%\def\backx{\overset{\leftarrow}{x}}
\def\backX{\overleftarrow{X}}
%\def\backpi{\overset{\leftarrow}{\mathbf{x}}}
\def\Zalt{Z^{\scriptscriptstyle\,\square}}
\def\Zalttil{\wt Z^{\scriptscriptstyle\,\square}}
\def\digamf{\Psi_0} %digamma function 
\def\tmaxigamf{\Psi_1} %trigamma function 
\def\funct lp{L} %a function needed
\def\funct lpbar{\bar L} %a function needed

\def\note#1{{\color{blue}{\bf(}#1{\bf)}}}
\def\pfnote#1{{\color{red}{\bf((} #1 {\bf))}}}
%\def\note#1{{\color{nicos-red}{\bf((} #1 {\bf))}}}
\def\Fnote#1{{\color{orange}{\bf((} #1 {\bf))}}}

%Firas' notation
\font \mymathbb = bbold10 at 11pt
%\newcommand{\one}{\mbox{\mymathbb{1}}}

\def\range{\mathcal R}
\def\Uset{\mathcal U}
\def\Diff{\mathcal D}
\def\EP{\mathcal E}
\def\EPlim{{\widehat{\mathcal E}}}
%\def\G{\mathcal G}
\def\K{\mathcal K}
\def\L{\mathcal L}
\def\cV{\mathcal V}
%\def\Yc{{\check Y}}
\def\Yc{{\w}}
\def\Y{Y}
\def\necorner{{{}_\urcorner}}
\def\swcorner{{{}^\llcorner}}
\def\Xexit{{M^{\cS}}}   %exit point from x-axis
\def\xexit{{m^{\cS}}}   %exit point from x-axis
\def\yexit{{n^{\cW}}}   %exit point from y-axis
%\def\dxexit{{m^{*,\swcorner}}  \def\dyexit{{n^{*,\swcorner}}}    %their duals
\def\xentrance{{m^{\cN}}}   %entrance point to x-boundary
\def\yentrance{{n^{\cE}}}   %entrance point  to y-boundary
\def\rect{{\mathfrak R}}
%\def\gne{G^{\textrm{\tiny{NE}},\xi}}
\def\gne{\wh G^{(\xi)}}
\def\Yh{{\wh\Y}}
\def\gpp{g}%{{g_{\text{pp}}}}
\def\gpl{{g_{\text{pl}}}}
\def\gppa{\gamma}
\def\Ga{G^{\xi}}
\def\Gsw{G}
%\def\Gne{\wh G}
\def\Ib{I^{\tiny\text{bulk}}}
\def\f{f}
\def\sa{s_{\alpha}}



%Firas' notation
%\def\range{\mathcal R}
%\def\Uset{\mathcal U}
%\def\Dset{\mathcal D}
%\def\G{\mathcal G}
%\def\cA{\mathcal A}
%\def\K{\mathcal K}
%\def\L{\mathcal L}
%\def\Yc{{\check Y}}
%\def\Y{Y}
%\def\necorner{{{}_\urcorner}}
%\def\swcorner{{{}^\llcorner}}
%\def\xexit{{m^{\swcorner}}}   %exit point from x-axis
%\def\yexit{{n^{\swcorner}}}   %exit point from y-axis
%%\def\dxexit{{m^{*,\swcorner}}  \def\dyexit{{n^{*,\swcorner}}}    %their duals
%\def\xentrance{{m^{\necorner}}}   %entrance point to x-boundary
%\def\yentrance{{n^{\necorner}}}   %entrance point  to y-boundary
%\def\rect{{\mathfrak R}}
%\def\V{{V}}
%\def\Vw{V_0}   %%%% the part of the potential that depends only on \w 
\def\cA{{\mathcal A}}
\def\cB{{\mathcal B}}
%\def\NA{{\mathcal B_0}}
%\def\Zpl{Z}
%\def\Zpp{Z}
%\def\Gpl{G}
%\def\Gpp{G}
%%\def\gpp{g_{\text{\rm pp}}}
%%\def\gpl{g_{\text{\rm pl}}}
%\def\Lapl{\Lambda_{\text{\rm pl}}}
%\def\Lapp{\Lambda_{\text{\rm pp}}}
%\def\ri{{\mathrm{ri\,}}}
%\def\f{{f}} %flux
%%\def\gppa{{\bar g}_{\text{\rm pp}}}
%\def\gppa{{\gamma}}
%\def\amin{{\underline\alpha}}
%\def\amax{{\overline\alpha}}
%\def\nabmin{{\underline\nabla}}
%\def\nabmax{{\overline\nabla}}
%\def\h{{h}}
%\def\hmin{{\underline h}}
%\def\hmax{{\overline h}}
%\def\smin{{\underline s}}
%\def\smax{{\overline s}}
%\def\ximin{{\underline\xi}}
%\def\ximax{{\overline\xi}}
%\def\zetamin{{\underline\zeta}}
%\def\zetamax{{\overline\zeta}}
%
%\def\Bmin{{\underline B}}
%\def\Bmax{{\overline B}}
%\def\Fmin{{\underline F}}
%\def\Fmax{{\overline F}}
%\def\zhat{{\hat z}}
%\def\B{{B}}
%\def\b{{b}}
%\def\Bbar{{\bar\B}}
%\def\cE{{\mathcal E}}
%\def\bB{{\mathbf B}}
%\def\G{{\mathbb G}}
%\def\I{{I}}
%\def\J{{J}}
%\def\Yc{{\w}}
%\def\W{{W}} %%%%  Mai-Pra queueing notation 
%\def\S{{S}}
%\def\A{{A}}
%\def\D{{D}}
%\def\Wp{{\wt W}}
%\def\Sp{{\wt S}}
%\def\Ap{{\wt A}}
%\def\M{{\mathcal M}}
%\def\U{{U}}
%\def\Ombig{{\widehat\Omega}}
%\def\Pbig{{\widehat\P}}
%\def\Ebig{{\widehat\E}}
%\def\kSbig{{\widehat\kS}}
%\def\OBP{(\Omega, \kS, \P)} 
%\def\OBPbig{(\Ombig, \kSbig, \Pbig)} 
%\def\www{{\bar\w}}
%\def\PPP{{\overline\P}}
%\def\EEE{{\overline\E}}
%\def\Ommm{{\overline\Omega}}
%\DeclareMathOperator{\ex}{ex}
%\def\O{{\mathcal O}}
%

%%Nicos notation
%\def\Gsw{G^{\rm SW}}
%%\def\Gsw{\overline{G}\!\!\!\!\phantom{G}^{\rm SW}}
%\def\Gne{G^{\rm NE}}   \def\Bne{B^{\rm NE}}
%\def\Ine{I^{\rm NE}}
%\def\Jne{J^{\rm NE}}
%%\def\Ibulk{I^{\rm bulk}}
%\def\Ibulk{I}
%%\def\Jbulk{J^{\rm bulk}}
%\def\Jbulk{J}
%\def\In{I^{\rm N}}
%\def\Jn{J^{\rm N}}
%\def\Ie{I^{\rm E}}
%\def\Je{J^{\rm E}}
%\def\Ge{G^{\rm E}}
%\def\Gn{G^{\rm N}}
%\def\Ine{I^{\rm NE}}
%\def\Jne{J^{\rm NE}}
%%\font\sz=cmr4 at 4pt

%\def\gsw#1{G^{\rm SW, (#1)}}
%\def\gne#1{G^{\rm NE, (#1)}}
%\def\gn#1{G^{\rm N, (#1)}}
%\def\nI#1{I^{\rm N, (#1)}}
%\def\neI#1{I^{\rm NE, (#1)}}
%\def\nJ#1{J^{\rm N, (#1)}}
%\def\neJ#1{J^{\rm NE, (#1)}}
%
%
%%%%%%%%   competition interface  
%\def\cid{\xi_*}
%\def\Bci{B^*}
%\def\Bbarci{\bar B^*}
%%\def\cidm{\cid}
%\def\cidmin{\underline\xi_{^{\scriptstyle*}}}
%\def\cidmax{\overline\xi_*}
%\def\cidd{\tau}   %limit of c.i. 
%\def\wgt{w}

%%%%%Timo
%\def\pp{p}  %the moment hypothesis  
%\def\Ew{m_0}   %mean of \w_0
%\def\opc{\vec p_c} 
%\def\Saset{V}  %the northeast edge of the a-triangle 
%\def\cl{\cO} 
%
%\def\cla{\cO} 
%\def\clb{\cO} 
%\def\aaa{\ell}   %triangle size 
%\def\etamin{{\underline\eta}}
%\def\etamax{{\overline\eta}}
%

\def\pc{\vec p_c}
\def\cO{\mathcal O}

\def\deq{\overset{d}=} 
\def\dto{\overset{d}\to} 

%%%%%  from Firas-bultima  
\def\varphimin{\varphi^{{\text\rm{(l)}}}}
\def\varphimax{\varphi^{{\text\rm{(r)}}}}
\def\cidl{\cid^{\text\rm{(l)}}}
\def\cidr{\cid^{\text\rm{(r)}}}
\def\cidlmin{\cidmin^{\text\rm{(l)}}}
\def\cidrmin{\cidmin^{\text\rm{(r)}}}
\def\cidlmax{\cidmax^{\text\rm{(l)}}}
\def\cidrmax{\cidmax^{\text\rm{(r)}}}
\def\cTl{\cT^{\textrm{(l)}}}
\def\thetal{\theta_*^{\text\rm{(l)}}}
\def\thetar{\theta_*^{\text\rm{(r)}}}
%\def\Bcir{\overline B_*}
%\def\Bcil{\underline B_*}
\def\cT{\mathcal T}

\def\ttvar{\alpha}   %% a variable in a Laplace transform -- not sure what it should be in the end. 

%%%%%%%   Timo def's 2016-09-23 for new file on multiclass CGM  

\def\OFP{(\Omega, \cF, P)} \def\OSP{(\Omega, \kS, \P)}
\def\OSPTh{(\Omega, \kS, \P, \Theta)}
\def\backpi{\overleftarrow{\pi}} 
\def\backx{\overleftarrow{x}}
%\def\backx{\overset{\leftarrow}{x}}
\def\backX{\overleftarrow{X}}
%\def\backpi{\overset{\leftarrow}{\pi}}
\def\Zalt{Z^{\scriptscriptstyle\,\square}}
\def\Zalttil{\wt Z^{\scriptscriptstyle\,\square}}
\def\digamf{\psi_0} %digamma function 
\def\trigamf{\psi_1} %trigamma function 
\def\funct lp{L} %a function needed
\def\funct lpbar{\bar L} %a function needed


\def\Dop{D}    %%% D operator for departure process 
\def\Rop{R}  %% check weights or time in the back of the queue  
\def\Sop{S}    %%% S operator for sojourn time process 
\def\Daop{\cD}   %%n"bigger" operators 
\def\Taop{\cT}
\def\Saop{\cS} 
%\newcommand{\lzb}{[\![}   %left Z bracket 
%\newcommand{\rzb}{]\!]}   %right Z bracket 
\newcommand{\lzb}{\llbracket}   %left Z bracket 
\newcommand{\rzb}{\rrbracket}   %right Z bracket 

%%%%% scaled objects 

\newcommand\abullet{{\raisebox{2pt}{\scaleobj{0.4}{\bullet}}}}  %%%% smaller bullet to use inside functions 
\newcommand\bbullet{{\scaleobj{0.7}{\bullet}}} 
\newcommand\rbbullet{{\raisebox{1pt}{\scaleobj{0.7}{\bullet}}}} 
\newcommand\cbullet{{\scaleobj{0.6}{\bullet}}} 
\newcommand\rcbullet{{\raisebox{1pt}{\scaleobj{0.5}{\bullet}}}} 
\newcommand\rdbullet{{\raisebox{1pt}{\scaleobj{0.4}{\bullet}}}} 

\newcommand\bnearrow{{\raisebox{1pt}{\scaleobj{0.6}{\mathbf\nearrow}}}}   %% \nearrow for a superscript so it doesn't look ridiculously big 


\newcommand\bcdot{{\scaleobj{1.8}{\cdot}}}

%%%%%%%%%%%%%%  end scaled object 

\def\qedrm{\hfill$\triangle$} 

\definecolor{darkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{darkblue}{rgb}{0.0,0.0,0.3}
\definecolor{nicosred}{rgb}{0.65,0.1,0.1}
\definecolor{light-gray}{gray}{0.7}
 
%\RequirePackage{datetime} %comment out when arxiving or submitting
%\usepackage{filemod}

 \def\Bus{B}
 \def\Buse#1{B^{#1}}
\newcommand\Busv[3]{\overline B^{#1,#2}_{#3}}

\def\Xw{X}  %another letter for a weight 
\def\Yw{Y}  %another letter for a weight 
\def\Ywch{\wc\Yw}  %another letter for a weight 
 
%\def\caY{\cY^{\bnearrow}}  % a space of ordered n-tuples 
\def\caY{\cY}  % arrow removed to simplify notation. 


%%%%geodesics 
\def\bgeod#1#2{\mathbf b^{#1, #2}}
\def\bgeoda#1{\bgeod{\alpha}{#1}}
\def\bgeodru{\bgeod{\rho}{u}}   \def\bgeodrx{\bgeod{\rho}{x}}   \def\bgeodrz{\bgeod{\rho}{z}}
\def\bgeodr#1{\bgeod{\rho}{#1}}

\def\arrow#1#2{\mathbf a^{#1}_{#2}}
\def\arrowa#1{\arrow{\alpha}{#1}}
\def\arrowru{\arrow{\rho}{u}}   \def\arrowrx{\arrow{\rho}{x}}   \def\arrowrz{\arrow{\rho}{z}}
\def\arrowr#1{\arrow{\rho}{#1}}

\def\counta{\xi}    %%%  count "a",  just a name for a r.v. 

\def\paramb{\tau}   %% needed a parameter -- not sure what a good letter choice is. 

\def\qedex{\hfill$\triangle$}  %%% end of remark, definition and example 

\def\imi{\iota}   %%not sure if want i or \iota for imaginary unit.  imi=imag.i 
\def\imu{\mathbf i}   %% imaginary unit 
%\def\imua{\bold i}      %command \bold obsolete 
\def\imua{\mathbf i}    % Jan. 2016 seems to work the best.


